Verification of Data-aware Business Processes in the Presence of Ontologies

The meet up between data, processes and structural knowledge in modeling enterprise systems is a challenging task that has led to the study of combining formalisms from knowledge representation, database theory, and process management. To ensure system correctness, formal verification also comes into play and offers well-established techniques. In line with this, significant results have been obtained within the research on data-aware business processes (DABP), which studies the marriage between static and dynamic aspects of a system within a unified framework. Here, we investigate the verification of DABP in the presence of ontologies, and provide the following contributions: (1) We propose a formal framework called Golog-KABs (GKABs), by leveraging on the state of the art formalisms for DABP equipped with ontologies. GKABs enable us to specify semantically-rich DABP, where the system dynamics are specified using a high-level action language inspired by the Golog programming language. (2) We propose a parametric execution semantics for GKABs that is able to elegantly accommodate a plethora of inconsistency-aware semantics based on the well-known notion of repair, and this leads us to several variants of inconsistency-aware GKABs. (3) We enhance GKABs towards context-sensitive GKABs. (4) We introduce the so-called Alternating-GKABs that allow for a more fine-grained analysis over the systems. (5) We introduce a novel framework called Semantically-Enhanced Data-Aware Processes (SEDAPs) that, by utilizing ontologies, enable us to have a high-level conceptual view over the evolution of the underlying system. We also provide reductions for the verification of sophisticated first-order temporal properties over all of the settings above, and show that verification can be addressed using existing techniques developed for Data-Centric Dynamic Systems (a well-established DABP framework).

==> 0.setting/track-change.tex <==
%############################################################################
%Track Changes
%############################################################################
% Change tracking
\usepackage[normalem]{ulem} % to override default set by changes package
\ifdraft
  \usepackage{0.Setting/mychanges}
  \usepackage[colorinlistoftodos]{todonotes}
\else
  \usepackage[final]{0.Setting/mychanges}
  \usepackage[disable]{todonotes}
\fi
\setauthormarkup[right]{{\scriptsize[#1]}}
%% \setauthormarkup{\marginpar{#1}}
\definechangesauthor{AS}{red}
\definechangesauthor{DC}{blue}
%% Commands to use in latex source (where author is one of DC, EK, ...):
%% \deleted[author]{text}
%% \added[author]{text}
%% \replaced[author]{new text}{old text}
\newcommand{\asd}[1]{\deleted[AS]{#1}} %ario deleted
\newcommand{\asa}[1]{\added[AS]{#1}} %ario added
\newcommand{\asr}[2]{\replaced[AS]{#1}{#2}} %ario replaced

\newcommand{\dc}[1]{\todo[inline]{#1}}
%############################################################################




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> glyphtounicode-cmr.tex <==
%
% Copyright (c) 2008,  Han The Thanh <thanh@river-valley.org>
% Copyright (c) 2014,  Peter Selinger <selinger@mathstat.dal.ca>
%                      
%  This file may be distributed and/or modified under the conditions
%  of the LaTeX Project Public License, either version 1.2 of this
%  license or (at your option) any later version.  The latest version
%  of this license is in:
%    
%    http://www.latex-project.org/lppl.txt
%    
%  and version 1.2 or later is part of all distributions of LaTeX
%  version 1999/12/01 or later.
%
% Changes:
% 2014/08/11: PS1 - mapped most glyphs to existing Unicode code points.
% 2014/08/11: PS1 - added mappings for the xyatip and xybtip fonts.

%% Glyphs from the cmex fonts:

\pdfglyphtounicode{angbracketleftBig}{27E8}
\pdfglyphtounicode{angbracketleftBigg}{27E8}
\pdfglyphtounicode{angbracketleftbig}{27E8}
\pdfglyphtounicode{angbracketleftbigg}{27E8}
\pdfglyphtounicode{angbracketrightBig}{27E9}
\pdfglyphtounicode{angbracketrightBigg}{27E9}
\pdfglyphtounicode{angbracketrightbig}{27E9}
\pdfglyphtounicode{angbracketrightbigg}{27E9}
\pdfglyphtounicode{arrowbt}{2193}
\pdfglyphtounicode{arrowdblbt}{21D3}
\pdfglyphtounicode{arrowdbltp}{21D1}
\pdfglyphtounicode{arrowhookleft}{21AA}
\pdfglyphtounicode{arrowhookright}{21A9}
\pdfglyphtounicode{arrowtp}{2191}
\pdfglyphtounicode{arrowvertex}{23D0}
\pdfglyphtounicode{arrowvertexdbl}{ED12}
\pdfglyphtounicode{backslashBig}{005C}
\pdfglyphtounicode{backslashBigg}{005C}
\pdfglyphtounicode{backslashbig}{005C}
\pdfglyphtounicode{backslashbigg}{005C}
\pdfglyphtounicode{braceex}{23AA}
\pdfglyphtounicode{bracehtipdownleft}{ED17}
\pdfglyphtounicode{bracehtipdownright}{ED18}
\pdfglyphtounicode{bracehtipupleft}{ED19}
\pdfglyphtounicode{bracehtipupright}{ED1A}
\pdfglyphtounicode{braceleftBig}{007B}
\pdfglyphtounicode{braceleftBigg}{007B}
\pdfglyphtounicode{braceleftbig}{007B}
\pdfglyphtounicode{braceleftbigg}{007B}
\pdfglyphtounicode{braceleftbt}{23A9}
\pdfglyphtounicode{braceleftmid}{23A8}
\pdfglyphtounicode{bracelefttp}{23A7}
\pdfglyphtounicode{bracerightBig}{007D}
\pdfglyphtounicode{bracerightBigg}{007D}
\pdfglyphtounicode{bracerightbig}{007D}
\pdfglyphtounicode{bracerightbigg}{007D}
\pdfglyphtounicode{bracerightbt}{23AD}
\pdfglyphtounicode{bracerightmid}{23AC}
\pdfglyphtounicode{bracerighttp}{23AB}
\pdfglyphtounicode{bracketleftBig}{005B}
\pdfglyphtounicode{bracketleftBigg}{005B}
\pdfglyphtounicode{bracketleftbig}{005B}
\pdfglyphtounicode{bracketleftbigg}{005B}
\pdfglyphtounicode{bracketleftbt}{23A3}
\pdfglyphtounicode{bracketleftex}{23A2}
\pdfglyphtounicode{bracketlefttp}{23A1}
\pdfglyphtounicode{bracketrightBig}{005D}
\pdfglyphtounicode{bracketrightBigg}{005D}
\pdfglyphtounicode{bracketrightbig}{005D}
\pdfglyphtounicode{bracketrightbigg}{005D}
\pdfglyphtounicode{bracketrightbt}{23A6}
\pdfglyphtounicode{bracketrightex}{23A5}
\pdfglyphtounicode{bracketrighttp}{23A4}
\pdfglyphtounicode{ceilingleftBig}{2308}
\pdfglyphtounicode{ceilingleftBigg}{2308}
\pdfglyphtounicode{ceilingleftbig}{2308}
\pdfglyphtounicode{ceilingleftbigg}{2308}
\pdfglyphtounicode{ceilingrightBig}{2309}
\pdfglyphtounicode{ceilingrightBigg}{2309}
\pdfglyphtounicode{ceilingrightbig}{2309}
\pdfglyphtounicode{ceilingrightbigg}{2309}
\pdfglyphtounicode{circledotdisplay}{2A00}
\pdfglyphtounicode{circledottext}{2A00}
\pdfglyphtounicode{circlemultiplydisplay}{2A02}
\pdfglyphtounicode{circlemultiplytext}{2A02}
\pdfglyphtounicode{circleplusdisplay}{2A01}
\pdfglyphtounicode{circleplustext}{2A01}
\pdfglyphtounicode{contintegraldisplay}{222E}
\pdfglyphtounicode{contintegraltext}{222E}
\pdfglyphtounicode{coproductdisplay}{2210}
\pdfglyphtounicode{coproducttext}{2210}
\pdfglyphtounicode{floorleftBig}{230A}
\pdfglyphtounicode{floorleftBigg}{230A}
\pdfglyphtounicode{floorleftbig}{230A}
\pdfglyphtounicode{floorleftbigg}{230A}
\pdfglyphtounicode{floorrightBig}{230B}
\pdfglyphtounicode{floorrightBigg}{230B}
\pdfglyphtounicode{floorrightbig}{230B}
\pdfglyphtounicode{floorrightbigg}{230B}
\pdfglyphtounicode{hatwide}{02C6}
\pdfglyphtounicode{hatwider}{02C6}
\pdfglyphtounicode{hatwidest}{02C6}
\pdfglyphtounicode{integraldisplay}{222B}
\pdfglyphtounicode{integraltext}{222B}
\pdfglyphtounicode{intersectiondisplay}{22C2}
\pdfglyphtounicode{intersectiontext}{22C2}
\pdfglyphtounicode{logicalanddisplay}{22C0}
\pdfglyphtounicode{logicalandtext}{22C0}
\pdfglyphtounicode{logicalordisplay}{22C1}
\pdfglyphtounicode{logicalortext}{22C1}
\pdfglyphtounicode{mapsto}{21A6}
\pdfglyphtounicode{parenleftBig}{0028}
\pdfglyphtounicode{parenleftBigg}{0028}
\pdfglyphtounicode{parenleftbig}{0028}
\pdfglyphtounicode{parenleftbigg}{0028}
\pdfglyphtounicode{parenleftbt}{239D}
\pdfglyphtounicode{parenleftex}{239C}
\pdfglyphtounicode{parenlefttp}{239B}
\pdfglyphtounicode{parenrightBig}{0029}
\pdfglyphtounicode{parenrightBigg}{0029}
\pdfglyphtounicode{parenrightbig}{0029}
\pdfglyphtounicode{parenrightbigg}{0029}
\pdfglyphtounicode{parenrightbt}{23A0}
\pdfglyphtounicode{parenrightex}{239F}
\pdfglyphtounicode{parenrighttp}{239E}
\pdfglyphtounicode{productdisplay}{220F}
\pdfglyphtounicode{producttext}{220F}
\pdfglyphtounicode{radicalBig}{221A}
\pdfglyphtounicode{radicalBigg}{221A}
\pdfglyphtounicode{radicalbig}{221A}
\pdfglyphtounicode{radicalbigg}{221A}
\pdfglyphtounicode{radicalbt}{221A}
\pdfglyphtounicode{radicaltp}{ED6A}
\pdfglyphtounicode{radicalvertex}{ED6B}
\pdfglyphtounicode{slashBig}{002F}
\pdfglyphtounicode{slashBigg}{002F}
\pdfglyphtounicode{slashbig}{002F}
\pdfglyphtounicode{slashbigg}{002F}
\pdfglyphtounicode{summationdisplay}{2211}
\pdfglyphtounicode{summationtext}{2211}
\pdfglyphtounicode{tie}{2040}
\pdfglyphtounicode{tildewide}{02DC}
\pdfglyphtounicode{tildewider}{02DC}
\pdfglyphtounicode{tildewidest}{02DC}
\pdfglyphtounicode{uniondisplay}{22C3}
\pdfglyphtounicode{unionmultidisplay}{2A04}
\pdfglyphtounicode{unionmultitext}{2A04}
\pdfglyphtounicode{unionsqdisplay}{2A06}
\pdfglyphtounicode{unionsqtext}{2A06}
\pdfglyphtounicode{uniontext}{22C3}
\pdfglyphtounicode{vextenddouble}{ED79}
\pdfglyphtounicode{vextendsingle}{23D0}

%% Glyphs from the cmr fonts:

\pdfglyphtounicode{suppress}{EB61}

%% Glyphs from the lasy fonts:

%% Note: unfortunately, some other fonts, such as line and xydash,
%% also use glyphs names a0...a127, but for different glyphs.

\pdfglyphtounicode{a1}{25C1}
\pdfglyphtounicode{a2}{22B4}
\pdfglyphtounicode{a3}{25B7}
\pdfglyphtounicode{a4}{22B5}
\pdfglyphtounicode{a40}{02C2}
\pdfglyphtounicode{a41}{02C3}
\pdfglyphtounicode{a42}{2303}
\pdfglyphtounicode{a43}{2304}
\pdfglyphtounicode{a48}{2127}
\pdfglyphtounicode{a49}{22C8}
\pdfglyphtounicode{a50}{25A1}
\pdfglyphtounicode{a51}{25C7}
\pdfglyphtounicode{a58}{2053}
\pdfglyphtounicode{a59}{219D}
\pdfglyphtounicode{a60}{228F}
\pdfglyphtounicode{a61}{2290}

%% Glyphs from the xyatip and xybtip fonts fonts of the XYPic package.
%% They denote half arrow tips pointing in various directions.  We map
%% them to Unicode arrows pointing in approximately the same
%% direction, in increments of 45 degrees.

\pdfglyphtounicode{d0}{2199}
\pdfglyphtounicode{d1}{2199}
\pdfglyphtounicode{d2}{2199}
\pdfglyphtounicode{d3}{2199}
\pdfglyphtounicode{d4}{2199}
\pdfglyphtounicode{d5}{2199}
\pdfglyphtounicode{d6}{2199}
\pdfglyphtounicode{d7}{2193}
\pdfglyphtounicode{d8}{2193}
\pdfglyphtounicode{d9}{2193}
\pdfglyphtounicode{d10}{2193}
\pdfglyphtounicode{d11}{2193}
\pdfglyphtounicode{d12}{2193}
\pdfglyphtounicode{d13}{2193}
\pdfglyphtounicode{d14}{2193}
\pdfglyphtounicode{d15}{2193}
\pdfglyphtounicode{d16}{2193}
\pdfglyphtounicode{d17}{2193}
\pdfglyphtounicode{d18}{2193}
\pdfglyphtounicode{d19}{2193}
\pdfglyphtounicode{d20}{2193}
\pdfglyphtounicode{d21}{2193}
\pdfglyphtounicode{d22}{2193}
\pdfglyphtounicode{d23}{2193}
\pdfglyphtounicode{d24}{2198}
\pdfglyphtounicode{d25}{2198}
\pdfglyphtounicode{d26}{2198}
\pdfglyphtounicode{d27}{2198}
\pdfglyphtounicode{d28}{2198}
\pdfglyphtounicode{d29}{2198}
\pdfglyphtounicode{d30}{2198}
\pdfglyphtounicode{d31}{2198}
\pdfglyphtounicode{d32}{2198}
\pdfglyphtounicode{d33}{2198}
\pdfglyphtounicode{d34}{2198}
\pdfglyphtounicode{d35}{2198}
\pdfglyphtounicode{d36}{2198}
\pdfglyphtounicode{d37}{2198}
\pdfglyphtounicode{d38}{2198}
\pdfglyphtounicode{d39}{2192}
\pdfglyphtounicode{d40}{2192}
\pdfglyphtounicode{d41}{2192}
\pdfglyphtounicode{d42}{2192}
\pdfglyphtounicode{d43}{2192}
\pdfglyphtounicode{d44}{2192}
\pdfglyphtounicode{d45}{2192}
\pdfglyphtounicode{d46}{2192}
\pdfglyphtounicode{d47}{2192}
\pdfglyphtounicode{d48}{2192}
\pdfglyphtounicode{d49}{2192}
\pdfglyphtounicode{d50}{2192}
\pdfglyphtounicode{d51}{2192}
\pdfglyphtounicode{d52}{2192}
\pdfglyphtounicode{d53}{2192}
\pdfglyphtounicode{d54}{2192}
\pdfglyphtounicode{d55}{2192}
\pdfglyphtounicode{d56}{2197}
\pdfglyphtounicode{d57}{2197}
\pdfglyphtounicode{d58}{2197}
\pdfglyphtounicode{d59}{2197}
\pdfglyphtounicode{d60}{2197}
\pdfglyphtounicode{d61}{2197}
\pdfglyphtounicode{d62}{2197}
\pdfglyphtounicode{d63}{2197}
\pdfglyphtounicode{d64}{2197}
\pdfglyphtounicode{d65}{2197}
\pdfglyphtounicode{d66}{2197}
\pdfglyphtounicode{d67}{2197}
\pdfglyphtounicode{d68}{2197}
\pdfglyphtounicode{d69}{2197}
\pdfglyphtounicode{d70}{2197}
\pdfglyphtounicode{d71}{2191}
\pdfglyphtounicode{d72}{2191}
\pdfglyphtounicode{d73}{2191}
\pdfglyphtounicode{d74}{2191}
\pdfglyphtounicode{d75}{2191}
\pdfglyphtounicode{d76}{2191}
\pdfglyphtounicode{d77}{2191}
\pdfglyphtounicode{d78}{2191}
\pdfglyphtounicode{d79}{2191}
\pdfglyphtounicode{d80}{2191}
\pdfglyphtounicode{d81}{2191}
\pdfglyphtounicode{d82}{2191}
\pdfglyphtounicode{d83}{2191}
\pdfglyphtounicode{d84}{2191}
\pdfglyphtounicode{d85}{2191}
\pdfglyphtounicode{d86}{2191}
\pdfglyphtounicode{d87}{2191}
\pdfglyphtounicode{d88}{2196}
\pdfglyphtounicode{d89}{2196}
\pdfglyphtounicode{d90}{2196}
\pdfglyphtounicode{d91}{2196}
\pdfglyphtounicode{d92}{2196}
\pdfglyphtounicode{d93}{2196}
\pdfglyphtounicode{d94}{2196}
\pdfglyphtounicode{d95}{2196}
\pdfglyphtounicode{d96}{2196}
\pdfglyphtounicode{d97}{2196}
\pdfglyphtounicode{d98}{2196}
\pdfglyphtounicode{d99}{2196}
\pdfglyphtounicode{d100}{2196}
\pdfglyphtounicode{d101}{2196}
\pdfglyphtounicode{d102}{2196}
\pdfglyphtounicode{d103}{2190}
\pdfglyphtounicode{d104}{2190}
\pdfglyphtounicode{d105}{2190}
\pdfglyphtounicode{d106}{2190}
\pdfglyphtounicode{d107}{2190}
\pdfglyphtounicode{d108}{2190}
\pdfglyphtounicode{d109}{2190}
\pdfglyphtounicode{d110}{2190}
\pdfglyphtounicode{d111}{2190}
\pdfglyphtounicode{d112}{2190}
\pdfglyphtounicode{d113}{2190}
\pdfglyphtounicode{d114}{2190}
\pdfglyphtounicode{d115}{2190}
\pdfglyphtounicode{d116}{2190}
\pdfglyphtounicode{d117}{2190}
\pdfglyphtounicode{d118}{2190}
\pdfglyphtounicode{d119}{2190}
\pdfglyphtounicode{d120}{2199}
\pdfglyphtounicode{d121}{2199}
\pdfglyphtounicode{d122}{2199}
\pdfglyphtounicode{d123}{2199}
\pdfglyphtounicode{d124}{2199}
\pdfglyphtounicode{d125}{2199}
\pdfglyphtounicode{d126}{2199}
\pdfglyphtounicode{d127}{2199}
\endinput

% Reference:
%
% http://codepoints.net/basic_latin
% 0028 0029 002F 005B 005C 005D 007B 007D
%
% http://codepoints.net/spacing_modifier_letters
% 02C2 02C3 02C6 02DC
%
% http://codepoints.net/general_punctuation
% 2040 2053
%
% http://codepoints.net/letterlike_symbols
% 2127
%
% http://codepoints.net/arrows
% 2190 2191 2192 2193 2196 2197 2198 2199 219D 21A6 21A9 21AA 21D1 21D3
%
% http://codepoints.net/mathematical_operators
% 220F 2210 2211 221A 222B 222E 228F 2290 22B4 22B5 22C0 22C1 22C2 22C3
% 22C8
%
% http://codepoints.net/miscellaneous_technical
% 2303 2304 2308 2309 230A 230B 239B 239C 239D 239E 239F 23A0 23A1 23A2
% 23A3 23A4 23A5 23A6 23A7 23A8 23A9 23AA 23AB 23AC 23AD 23D0
%
% http://codepoints.net/geometric_shapes
% 25A1 25B7 25C1 25C7
%
% http://codepoints.net/miscellaneous_mathematical_symbols-a
% 27E8 27E9
%
% http://codepoints.net/supplemental_mathematical_operators
% 2A00 2A01 2A02 2A04 2A06
%
% Private Use Area:
% EB61 ED12 ED17 ED18 ED19 ED1A ED6A ED6B ED79

%
%
% End of file 'glyphtounicode-cmr.tex
%

